Tor's Been KIST: A Case Study of Transitioning Tor Research to Practice

Most computer science research is aimed at solving difficult problems with a goal of sharing the developed solutions with the greater research community. For many researchers, a project ends when the paper is published even though a much broader impact could be achieved by spending additional effort to transition that research to real world usage. In this paper, we examine the opportunities and challenges in transitioning Tor research through a case study of deploying a previously proposed application layer socket scheduling policy called KIST into the Tor network. We implement KIST, simulate it in a 2,000-relay private Tor network using Shadow, deploy it on a Tor relay running in the public Tor network, and measure its performance impact. Confirming the results reported in prior research, we find that KIST reduces kernel outbound queuing times for relays and download times for low-volume or bursty clients. We also find that client and relay performance with KIST increases as network load and packet loss rates increase, although the effects of packet loss on KIST were overlooked in past work. Our implementation will be released as open-source software for inclusion in a future Tor release.

==> sections/discussion.tex <==
\section{Discussion and Lessons Learned} \label{sec:discussion}

In this section, we discuss some lessons that we learned throughout our case
study that we believe could generally apply to the Tor research community. We
first look at challenges we faced while evaluating our own work and then discuss
the difficulty of resolving the differences between the Tor developers'
priorities and ours with respect to implementing KIST.

\subsection{Evaluation Challenges}

For testing the KIST socket scheduling policy, we primarily performed ongoing
Shadow network simulations. Small networks allowed rapid development iteration
during implementation while large networks produced data that is easier to compare to
the live Tor network. The control that simulation gave us was instrumental in our
ability to continuously test KIST. Simulation allowed us to vary network parameters such as packet
loss, latency, and link speed to understand how the AMAP and KIST policies react to
different network conditions, and we could control and observe how every client
circuit was built. The accuracy of Tor simulations increase as the size of the network
approaches the size of the public Tor network. However, scaling up to many thousands
of Tor clients and relays introduces computing resource challenges. Our largest simulations from \S\ref{sec:simeval:net} consumed 1 TB of RAM and took 8 days to simulate 45 minutes of time.
While we have the hardware resources to handle these large simulations, other researchers may not and therefore compromises in simulation accuracy may need to be made.
We also went through a lengthy process to ensure that the fidelity of Shadow's TCP
implementation adequately modeled the Linux kernel's such that our results
would be comparable. As previously discussed, our Shadow results are promising,
but we also wanted to run a live relay in order to be able to measure KIST's performance characteristics in the wild.

While our Shadow simulation results should be reproducible, our live network
throughput results are not: the constantly changing topology and background
traffic of the public Tor network introduces uncertainty that we can draw
meaningful conclusions about how KIST affects relay throughput from our live
network results, even after 6 weeks of data collection. The consensus weight of
our relay varied between about 0.07\% and 0.13\% during the course of our data
collection and one of the Tor network bandwidth scanners that measures relays
went down\cite{list-bwauth}, causing many relay operators to notice significant
changes in their bandwidth usage. Our lack of control over the rest of the Tor
network makes attributing throughput variance to our changes difficult. Even so,
we believe that our live relay results in \S\ref{sec:neteval} show that KIST is
\textit{at least} no worse than the AMAP socket scheduling policy.

\subsection{Differing Priorities}

The Tor developers are always busy with bug fixes and Tor's own feature goals.
Researchers are no different. If they are judged primarily by quality and
quantity of papers they author, there is little motivation for them to spend the
time to transition their code from a working prototype to clean, compatible, and
implementable code in Tor. Periodic conversations
with Tor developers occasionally led to additional prototypes but never a
finished product that could be called KIST. Tor developers implemented the
global socket scheduler as recommended and attempted a KIST-like socket
scheduling policy; however, the resulting AMAP policy has underlying issues
preventing it from ever acting like KIST even if its parameters had been tuned
to be more than just backwards compatible. Another Tor developer worked briefly
on implementing per-socket write limits for KIST but never got it working.

The passage of time also hindered KIST's ability to make it into Tor. Version
\texttt{0.2.3.25} was the latest stable version of Tor when Jansen \etal wrote
the original KIST prototype. Global scheduling and the AMAP socket scheduling
policy were added in version \texttt{0.2.6.2-alpha}, by which time significant
changes in Tor's code base made the original prototype obsolete. We started
implementing the KIST socket scheduling policy against Tor stable version
\texttt{0.2.8.10} and are working with Tor to have it merged into the
\texttt{0.3.2} stable release series. As researchers, we prefer to pick a
baseline version to compare against and to keep using that version for the
duration of a project in order to produce consistent results. Tor, on the other
hand, avoids merging code written for an outdated version. As we transition into
merging our code into Tor, do we need to rerun our experiments? Some of them are
expensive and take a long time to run. Are experiments using code that is one
stable version out-of-date any better than two versions out-of-date? Early and
consistent discussions with Tor developers may help to answer these and other questions.

%\matt{no mention of 
%(i) how will deployment get graduate students to their degree faster?
%(ii) not security vuln, so not high priority
%}


